Accurate battery lifetime prediction across diverse aging conditions with deep learning

Accurately predicting the lifetime of battery cells in early cycles holds tremendous value for battery research and development as well as numerous downstream applications. This task is rather challenging because diverse conditions, such as electrode materials, operating conditions, and working environments, collectively determine complex capacity-degradation behaviors. However, current prediction methods are developed and validated under limited aging conditions, resulting in questionable adaptability to varied aging conditions and an inability to fully benefit from historical data collected under different conditions. Here we introduce a universal deep learning approach that is capable of accommodating various aging conditions and facilitating effective learning under low-resource conditions by leveraging data from rich conditions. Our key finding is that incorporating inter-cell feature differences, rather than solely considering single-cell characteristics, significantly increases the accuracy of battery lifetime prediction and its cross-condition robustness. Accordingly, we develop a holistic learning framework accommodating both single-cell and inter-cell modeling. A comprehensive benchmark is built for evaluation, encompassing 401 battery cells utilizing 5 prevalent electrode materials across 168 cycling conditions. We demonstrate remarkable capabilities in learning across diverse aging conditions, exclusively achieving 10% prediction error using the first 100 cycles, and in facilitating low-resource learning, almost halving the error of single-cell modeling in many cases. More broadly, by breaking the learning boundaries among different aging conditions, our approach could significantly accelerate the development and optimization of lithium-ion batteries.

==> sections/mechanism.tex <==
\begin{figure*}[!t]
    \includegraphics[width=\linewidth]{images/final_fig5.pdf}
    \caption{Ablation studies. \textbf{a}: Enhanced predictive performance necessiates the inclusion of the complete voltage and current signals, as well as their interactions, from both charging and discharging stages.
    % \textbf{b}: Intra-cell difference model is prune to overfitting while inter-cell difference model and DCBLP exhibit robust convergence.
    \textbf{b}: Leveraging the joint training of IntraCD and InterCD branches, BatDiff achieves superior performance than the ensemble of IntraCD and InterCD models.
    % \textbf{c}: Comparison of transfer- and InterCD-based methods that utilize historical data to enhance the prediction of new battery types. Employing the InterCD-based method to explicitly model battery interrelations leads to a substantial improvement in prediction performance for new battery types.
    }
    \label{fig:ablation}
\end{figure*}

\section{Mechanism of BatDiff}
% \subsection{InterCD Enhances Lifetime Prediction of New Batteries through Efficient Historical Battery Utilization}
% \subsection{BatDiff Effectively Combines InterCD and IntraCD}
% \subsection{BatDiff Benefits from Diverse Input Signals}

Here we conduct further ablation experiments to study the mechanism of BatDiff.

% \figurename~\ref{fig:ablation}b illustrates the convergence of IntraCD, InterCD, and DCBLP during training on \texttt{MIX-100}.
% We observed that the IntraCD model quickly reaches a low error at the 200-th epoch but then starts to overfit.
% As training progresses, the variance between different seeds of IntraCD gradually intensifies and the models continue to diverge.
% In practice, without additional validation samples for early stopping due to the data scarcity issue, the IntraCD-based methods demonstrate poor robustness and are very sensitive to initialization.
% In contrast, the InterCD-based method gradually converge during training without overfitting, irrespective of the random seed employed.
% This highlights the robustness of the InterCD-based method, although its final regression error is slightly larger than the lowest error of the IntraCD-based method.
% Owing to the co-training of the both branches, DCBLP combines the advantages of both branches and robustly converges to a more accurate solution.

\figurename~\ref{fig:ablation}\textbf{a} compares the predictive performance of different BatDiff branches.
Across all datasets, IntraCD exhibit the highest error and variance.
The InterCD-based model shows good robustness with lower variance across all datasets, yet its prediction accuracy is slightly lower than that of the IntraCD on some datasets, as its predictions are implicitly derived through the reference cells.
The ensemble of the two separately trained branches obtains better performance on \texttt{HUST} and \texttt{MIX-100}, yet on other datasets it inherits the flaws of either branch, resulting in higher variance or suboptimal accuracy.
BatDiff achieved the most robust and precise lifetime estimation across all datasets, demonstrating that through the co-training with shared prediction layers, the model better integrates the strength of both branches and yields the strongest predictive performance.
\figurename~S7 shows their convergence curves, confirming that IntraCD-based model can easily overfit while InterCD converges robostly.

\figurename~\ref{fig:ablation}\textbf{b} displays the performance of BatDiff when using a subset of the six capacity-indexed features.
It's evident that all six features play a crucial role in achieving improved predictive performance. 
The current-based features can lead to high variance and large errors, yet they are indispensable for the extreme early prediction scenarios in \texttt{MIX-20}.
The voltage- and discharge-based features demonstrate strong performance across all datasets.
Merging voltage and current features from both charge and discharge stages results in enhanced performance, with the best outcomes achieved by employing all six features.

We further investigated the mechanism of InterCD in a realistic battery testing scenario where we need to use the historical battery data to boost the prediction of a new battery type.
We divided batteries in \texttt{MIX-100} into four categories according to the electrode material, resulting in 225 LFP cells, 32 lithium cobalt oxides (LCO) cells, 61 lithium nickel manganese cobalt oxides (NMC) cells, and 19 lithium nickel cobalt aluminium oxides (NCA) cells.
We assumed that the full life cycle data of the LFP batteries were known and employed them to assist the prediction of the other three types of batteries.
Among these target types, we randomly sample a small fraction of batteries as training cells.
The fraction is kept within 20\% to mimic the limited testing cost in practice.
We considered two learning enhancement methods.
The first method was pre-training on LFP data and then fine-tuning on the target batteries, a typical transfer learning paradigm.
The second method was to learn an InterCD model directly on the LFP-target battery pairs, and then ensemble with the IntraCD model trained on the limited target cells.

% \figurename~\ref{fig:ablation}\textbf{c} shows the comparison results on these three types of batteries.
% Compared to transfer learning, the InterCD-based model demonstrates a lower average error and significantly smaller variances on all three types of batteries.
% Notably, the performance gap between the transfer-learning- and InterCD-based methods increases as we use less target cells.
% InterCD-based model even decreased the error by half compared to transfer learning when using only 5\% of the data for training.
% This indicates that InterCD can make more effective use of existing data and thus is less sensitive to data scarcity issues.
% In practice, InterCD-based methods such as BatDiff can significantly reduce testing costs while ensuring prediction accuracy.
% This feature will greatly benefit downstream tasks, such as optimizing battery charging and discharging strategies or electrode materials.


==> sections/results.tex <==
\begin{figure*}[!t]
    \includegraphics[width=\linewidth]{images/fig2_new.pdf}
    \caption{Visualization of datasets. \textbf{a}: The coverage of the dataset employed in this work significantly surpasses that of previous undertakings, namely the NE\cite{NE}, CLO\cite{CLO}, SNL\cite{SNL}, HUST\cite{HUST}, and CALCE\cite{CALCE1,CALCE2,CALCE3}. \textbf{b}: A visualization of the capacity degradation with respect to the cycles for all the cells. The curves are normalized by their nominal capacities. The first $1500$ and $100$ cycles are shown. The degradation patterns are highly non-linear and are difficult to distinguish in the first $100$ cycles.}
    \label{fig:dataset}
\end{figure*}

% \begin{table*}[!t]
% \footnotesize
% \begin{tabular}{lllllllllllll}
% \toprule
% {\multirow{2}{*}{Method}} & \multicolumn{2}{c}{MATR-1} & \multicolumn{2}{c}{MATR-2} & \multicolumn{2}{c}{MATR-full} & \multicolumn{2}{c}{HUST} & \multicolumn{2}{c}{MIX-20} & \multicolumn{2}{c}{MIX-100} \\
% {} &    RMSE & MAPE(\%) &     RMSE & MAPE(\%) &      RMSE & MAPE(\%) &    RMSE & MAPE(\%) &     RMSE & MAPE(\%) &    RMSE & MAPE(\%) \\
% \midrule
% Training Mean                 &     399 &      28 &      511 &      36 &       331 &      31 &     420 &      18 &      593 &     102 &     573 &      59 \\
% \midrule
% ``Variance'' Model\cite{NE}        &     138 &      15 &      196 &      12 &       179 &      17 &     398 &      17 &      601 &      95 &     521 &      39 \\
% ``Discharge'' Model\cite{NE}       &      \underline{86} &       \underline{8} &      \underline{173} &      \underline{11} &       144 &      14 &     \underline{322} &      \underline{14} &  >2000 &    >100 &    1743 &      47 \\
% ``Full'' Model\cite{NE}            &     100 &      11 &      214 &      12 &       \underline{139} &      14 &     335 &      14 &      441 &      53 &     331 &      22 \\
% Ridge Regression\cite{attia2021statistical}      &     125 &      13 &      188 &      11 &       178 &      13 &    1047 &      36 &      806 &     150 &     395 &      30 \\
% PCR\cite{attia2021statistical}                   &     100 &      11 &      176 &      11 &       173 &      13 &     435 &      19 &      701 &      78 &     384 &      28 \\
% PLSR\cite{attia2021statistical}                  &      97 &      10 &      193 &      11 &       168 &      13 &     431 &      18 &      543 &      77 &     371 &      26 \\
% SVM Regression        &     140 &      15 &      300 &      18 &       145 &      \underline{11} &     344 &      16 &      438 &      46 &     257 &      18 \\
% Random Forest\cite{attia2021statistical}         &     140 &      15 &      202 &      11 &       203 &      16 &     348 &      16 &      \underline{288} &      \underline{31} &     \underline{211} &      \underline{14} \\
% \midrule
% MLP\cite{attia2021statistical}                   &   162±7 &    12±0 &    207±4 &    11±0 &     165±5 &    12±1 &   444±5 &    18±1 &   532±25 &    61±6 &  455±37 &    27±1 \\
% LSTM                  &  123±11 &    12±2 &   226±36 &    14±2 &    200±21 &    14±1 &  442±32 &    20±1 &   417±62 &    37±7 &  266±11 &    15±1 \\
% CNN\cite{attia2021statistical}                   &  115±96 &     9±6 &  237±107 &    17±8 &    223±72 &    15±3 &  445±35 &    21±1 &  785±132 &    41±4 &  261±38 &    15±1 \\
% \midrule
% % InterCD &    73±3 &     7±0 &   260±13 &    17±1 &     109±7 &    10±1 &  265±10 &    10±1 &   210±15 &    18±1 &  181±13 &    12±1 \\
% % BatDiff                 &    \textbf{59±2} &     \textbf{6±0} &   \textbf{163±12} &    \textbf{11±1} &      \textbf{85±8} &     \textbf{7±1} &   \textbf{264±9} &    \textbf{10±1} &   \textbf{201±18} &    \textbf{18±1} &   \textbf{158±7} &    \textbf{10±0} \\
% \texttt{BatLiNet} (ours) &    \textbf{59±2} &     \textbf{6±0} &   \textbf{163±12} &    \textbf{11±1} &      \textbf{85±8} &     \textbf{7±1} &   \textbf{264±9} &    \textbf{10±1} &   \textbf{201±18} &    \textbf{18±1} &   \textbf{158±7} &    \textbf{10±0} \\
% \bottomrule
% \end{tabular}
% \caption{Comparison results with baseline methods. We employ bold font to emphasize the best-performing method and utilize underlines to denote the second-best baselines. For neural-network-based methods, we report the mean and standard deviation of eight random seeds.}
% \label{tab:main}
% \end{table*}

\begin{table*}[!t]
% \footnotesize
\small
\begin{tabular}{lllllllllll}
\toprule
{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{MATR-1} & \multicolumn{2}{c}{MATR-2}  & \multicolumn{2}{c}{HUST} & \multicolumn{2}{c}{MIX-100} & \multicolumn{2}{c}{MIX-20} \\
{} &    RMSE & MAPE(\%) &     RMSE & MAPE(\%) &      RMSE & MAPE(\%) &     RMSE & MAPE(\%) &    RMSE & MAPE(\%) \\
\midrule
Training Mean                 &     399 &      28 &      511 &      36 &      420 &      18 &      573 &     59 &     593 &      102 \\
\midrule
``Variance'' Model\cite{NE}        &     138 &      15 &      196 &      12 &        398 &      17 &      521 &      39 &     601 &      95 \\
``Discharge'' Model\cite{NE}       &      \underline{86} &       \underline{8} &      \underline{173} &      \underline{11} &       \underline{322} &      \underline{14} &  1743 &    47 &    >2000 &      >100 \\
``Full'' Model\cite{NE}            &     100 &      11 &      214 &      12 &         335 &      14 &      331 &      22 &     441 &      53 \\
Ridge Regression\cite{attia2021statistical}      &     125 &      13 &      188 &      11 &       1047 &      36 &      395 &     30 &     806 &      150 \\
PCR\cite{attia2021statistical}                   &     100 &      11 &      176 &      11 &      435 &      19 &      384 &      28 &     701 &      78 \\
PLSR\cite{attia2021statistical}                  &      97 &      10 &      193 &      11 &      431 &      18 &      371 &      26 &     543 &      77 \\
SVM Regression        &     140 &      15 &      300 &      18 &     344 &      16 &      257 &      18 &     438 &      46 \\
Random Forest\cite{attia2021statistical}         &     140 &      15 &      202 &      11 &      348 &      16 &      \underline{211} &      \underline{14} &     \underline{288} &      \underline{31} \\
\midrule
MLP\cite{attia2021statistical}                   &   162±7 &    12±0 &    207±4 &    11±0 &   444±5 &    18±1 &  455±37 &    27±1 &   532±25 &    61±6\\
LSTM                  &  123±11 &    12±2 &   226±36 &    14±2 &    442±32 &    20±1 &   266±11 &    15±1 & 417±62 &    37±7 \\
CNN\cite{attia2021statistical}                   &  115±96 &     9±6 &  237±107 &    17±8 &    445±35 &    21±1  &  261±38 &    15±1 &  785±132 &    41±4 \\
\midrule
\texttt{BatLiNet} (ours) &    \textbf{59±2} &     \textbf{6±0} &   \textbf{163±12} &    \textbf{11±1} &    \textbf{264±9} &    \textbf{10±1} &   \textbf{158±7} &    \textbf{10±0} &   \textbf{201±18} &    \textbf{18±1}\\
\bottomrule
\end{tabular}
\caption{Comparison results with baseline methods. We employ bold font to emphasize the best-performing method and utilize underlines to denote the second-best baselines. For neural-network-based methods, we report the mean and standard deviation of eight random seeds.}
\label{tab:main}
\end{table*}

% \begin{figure*}[!t]
%     \includegraphics[width=0.8\linewidth]{images/fig2.5.pdf}
%     \caption{Visualization of comparison results. \textbf{a}: Performance of NN-based methods using different random seeds. CNN model exhibits larger variance than LSTM but sometimes achieves smaller errors. BatDiff is more accurate and robust to all baseline models. \textbf{b}: Prediction error for individual battery cells of \texttt{MIX-100} dataset. \textbf{c}: Cumulative absolute error plotted with respect to the fraction of test samples used from \texttt{MIX-100} dataset. Stronger models are those closer to the upper-left corner.}
%     \label{fig:comparison}
% \end{figure*}
\begin{figure*}[!t]
    \includegraphics[width=0.9\linewidth]{images/final_fig3.pdf}
    \caption{}
    \label{fig:seed_robustness}
\end{figure*}

\section{BatDiff Ensures Accurate Predictions across Aging Conditions}

We curated, to the best of our knowledge, all the existing battery data suitable for early battery life prediction to comprehensively evaluate our method in comparison with existing approaches.
Six distinct test datasets covering various of battery models and operating conditions are constructed for experimentation.

\texttt{MATR-1} and \texttt{MATR-2}~\cite{NE} consist of $123$ commercial 18650 lithium-ion phosphate/graphite (LFP) batteries.
All batteries share the same discharging protocol but are charged at different rates.
\texttt{MATR-2} requires the model to generalize to different charging protocols while the training and test dataset of \texttt{MATR-1} follow the same distribution.
We construct \texttt{MATR-full} that includes all the batteries from \texttt{MATR-1} and \texttt{MATR-2}, as well as additional $55$ LFP 18650 cells cycled with the optimized charging protocols~\cite{CLO} to assess how the model generalizes across diverse data batches obtained at different time points.
The \texttt{HUST} dataset~\cite{HUST} involves $77$ LFP batteries with a constant charging protocol but different discharge speeds.
All the cells in these four datasets belong to the same battery model.

Additionally, we collected batteries used in prior studies including CALCE~\cite{CALCE1,CALCE2,CALCE3}, HNEI~\cite{HNEI}, UL-PUR~\cite{ULPUR}, RWTH~\cite{RWTH} and SNL~\cite{SNL}.
By combining these batteries with \texttt{MATR-full} and \texttt{HUST}, we obtained a total collection of 401 batteries.
To evaluate the performance under different lifetime prediction scenarios, we developed two test datasets \texttt{MIX-20} and \texttt{MIX-100}.
In \texttt{MIX-20}, the models are required to predict the cycles before degradation to 90\% of the nominal capacity, using the data from only the first 20 cycles.
In \texttt{MIX-100}, the models predict the 80\% end of life point using data from the first 100 cycles.
Notably, batteries that had already degraded to the end of life during the early cycles were excluded in the experiments.

\figurename~\ref{fig:dataset}\textbf{a} shows that the collected dataset exhibits a more comprehensive coverage that goes beyond the confines of previous works.
\figurename~\ref{fig:dataset}\textbf{b} further visualizes the capacity degradation of the collected batteries in the first $1500$ and $100$ cycles of the batteries.
Here the long-term degradation is highly non-linear and demonstrates considerable variation among batteries.
In contrast, the degradation within the initial 100 cycles remains indiscernible for most batteries.
Such diverse and intricate characteristics require the model to capture and distinguish the degradation patterns caused by various factors for generalization.
% For more comprehensive details on dataset construction, please refer to the Supplementary Information.

Table~\ref{tab:main} presents the comparison results of the proposed methods against various baselines on these six datasets.
Employing only the InterCD method achieves superior performance on \texttt{MATR-1}, \texttt{MATR-full} and \texttt{HUST}.
This indicates that the model effectively captures the degradation patterns of the LFP cells under different charging and discharging protocols.
InterCD shows even larger performance advantage in comparison with the baselines on \texttt{MIX-20} and \texttt{MIX-100}.
This phenomenon arises due to the tendency of the IntraCD-based baselines to underfit or even diverge as they encounter an increasing variety of battery types.
In contrast, the InterCD adeptly captures the diverse degradation patterns, thus yielding more accurate predictions.
The InterCD method demonstrates a suboptimal performance of the InterCD method on \texttt{MATR-2}.
\figurename~S2 indicates the cause is that several battery cells with long lifespans resemble the electrical signals of batteries with much smaller lifetimes.
\figurename~S3 shows both IntraCD and InterCD underestimate the lifespans of these batteries, and InterCD makes bolder predictions due to their high similarity with short-lifespan batteries, as visualized by \figurename~S4.

With the joint training of IntraCD and InterCD branches, BatDiff further boosts the prediction performance over InterCD alone, leading to the lowest prediction errors on all datasets.
It is important to note that, no method prior to BatDiff has managed to consistently achieve optimal performance across all datasets.
BatDiff reduced the root mean square error (RMSE) over the second-best baselines by $31.4\%$, $5.8\%$, $38.8\%$, $18.0\%$, $30.2\%$, $25.11\%$ respectively on the six datasets.
BatDiff also achieved $\leq 18\%$ mean absolute percentage error (MAPE) on all datasets, meaning that BatDiff predicts relatively small errors for all cells under diverse prediction scenarios.
In contrast, the baseline methods occasionally produce $>30\%$ MAPE, rendering them unsuitable for general applications.

\figurename~\ref{fig:comparison}\textbf{a} demonstrates the comparison of deep models under different random seeds on the six datasets.
Among the baselines, the multi-layer perceptron (MLP) demonstrates modest prediction errors with the lowest variance on average.
The RMSE of the convolutional network (CNN) shows the largest variance, yet achieves the lowest errors in four datasets among the baselines. Note that CNN becomes the strongest baseline when using the optimal seeds~\cite{attia2021statistical}.
The long short term memory (LSTM) network achieves the best accuracy-variance trade-off.
BatDiff outperforms these baselines in both accuracy and robustness.
\figurename~\ref{fig:comparison}\textbf{b} displays the instance-level prediction errors of BatDiff on \texttt{MIX-100} dataset, where the absolute percentage error is lower than $20\%$ for $84.7\%$ cells. \figurename~\ref{fig:comparison}\textbf{c} plots the cumulative absolute error with respect to the fraction of test samples in \texttt{MIX-100} dataset. The error curves of the random forest (RF) and BatDiff initially coincide for the first approximately $50\%$ of test samples, after which the error of RF begins to escalate at a faster rate than that of BatDiff. This suggests that RF accurately captures the patterns within a subset of the samples, whereas BatDiff excels at capturing the patterns in the remaining portion. Finally, the consistent slope of the error growth curve for BatDiff signifies that BatDiff does not exhibit excessively large prediction errors for any batteries.

==> sections/results_save.tex <==
\section{Results}

\subsection{Deep Contrastive Battery Lifetime Prediction (DCBLP) Framework}

\begin{figure*}[!t]
    \includegraphics[width=\linewidth]{images/fig1_new.pdf}
    \caption{Inter-cell difference features and the deep contrastive battery lifetime prediction (DCBLP) framework. \textbf{a}: Illustration of intra- and inter-cell difference features. \textbf{b}: Both intra- and inter-cell difference features demonstrate a high correlation with the battery lifetime. \textbf{c}: The architecture of the DCBLP framework.}
    \label{fig:pipeline}
\end{figure*}

% In this article, we present a novel deep contrastive framework designed to tackle the task of predicting battery lifetime in general scenarios.
\figurename~\ref{fig:pipeline} illustrates the core ideas and the overall pipeline of this framework.
% At the core of the framework are two key concepts: the cross-difference feature space and the deep contrastive co-training of self- and cross-difference-based predictors.

% As shown in \figurename~\ref{fig:pipeline}a, previous methods rely on the \textit{inter-cell difference} (InterCD) features of voltage-capacity curves, utilizing a specific cycle of the target battery as the reference signal (upper \figurename~\ref{fig:pipeline}).
% The difference curves, derived by subtracting the reference cycle from the remaining cycles, demonstrate a strong correlation with the battery lifetime.
% However, such IntraCD-based methods fail to harness the information across diverse battery instances.
% As a result, they usually experience a suboptimal data utilization and are susceptible to overfitting in data-scarce scenarios.

\begin{figure*}[!t]
    \includegraphics[width=\linewidth]{images/fig2_new.pdf}
    \caption{Visualization of datasets. \textbf{a}: The coverage of the dataset employed in this work significantly surpasses that of previous undertakings. \textbf{b}: A visualization of the capacity degradation with respect to the cycles for all the cells. The curves are normalized by their nominal capacities. The first $1500$ and $100$ cycles are shown. The degradation patterns are highly non-linear and are difficult to distinguish in the first $100$ cycles.}
    \label{fig:dataset}
\end{figure*}

As shown in \figurename~\ref{fig:pipeline}a, previous methods rely on the \textit{inter-cell difference} (InterCD) features of voltage-capacity curves, utilizing a specific cycle of the target battery as the reference signal (upper \figurename~\ref{fig:pipeline}).
% The difference curves, derived by subtracting the reference cycle from the remaining cycles, demonstrate a strong correlation with the battery lifetime.
However, such IntraCD-based methods fail to harness the information across diverse battery instances.
As a result, they usually experience a suboptimal data utilization and are susceptible to overfitting in data-scarce scenarios.
In contrast, we propose the utilization of \textit{inter-cell difference} (InterCD) features to leverage the interrelation between batteries for accurate and robust lifetime prediction.
% First, for any given target battery, we calculate six capacity-indexed feature curves to encode the full information of its electrical behaviors (\figurename~\ref{fig:pipeline}a only displays the discharge voltage-capacity curves for clarity).
First, for any given target battery, we calculate six capacity-indexed feature curves as raw inputs, which includes 1-2) discharge current-capacity curve $I(Q_c)$ and voltage-capacity curve $V(Q_c)$, 3-4) charge current-capacity curve $I(Q_d)$ and voltage-capacity curve $V(Q_d)$, 5) differential voltage-capacity curve $V(Q_c) - V(Q_d)$ and 6) the resistance-capacity curve $\frac{V(Q_c)-V(Q_d)}{I(Q_c)-I(Q_d)}$. Please refer to the method section for more details.
% Here \figurename~\ref{fig:pipeline}a only displays the discharge voltage-capacity curves for clarity.
Second, we randomly sample a battery with a known lifetime from the training dataset as the reference cell and subtract its features from the corresponding cycles of the target cell.
Here, the capacity of each battery is normalized to $[0, 1]$ with respect to its nominal capacity in order to properly calculate the difference between distinct battery types.
The difference curves therefore encode the degradation information of both battery cells.
% Lower \figurename~\ref{fig:pipeline}b shows that these InterCD features also demonstrate a high correlation with the battery lifetime difference, which implies the lifetime of the target cell as the reference lifetime is known.
% In \figurename~\ref{fig:pipeline}c we demonstrated the InterCD voltage-capacity curves with different reference cells.
% When comparing batteries with equivalent electrode materials and operational conditions, the cross-difference feature curves closely resemble the self-difference curves.
% For batteries with distinct electrode materials, the cross-difference curves encompass the ageing patterns of both material types and reflect their variations in thermodynamics and kinetics.
% This allows us to utilize these cross-difference curves to forecast the lifetime difference of the two batteries.
% Consequently, the lifetime of the target cell can be ascertained by adding this prediction to the reference lifetime.

% \figurename~\ref{fig:pipeline}b visually demonstrates the direct relationship between V-Q curves and battery lifespan based on two different reference signals. The left side of Figure 2b illustrates the relationship between the variance of V-Q curves for self-difference and battery lifespan, where the reference signal is the V-Q curve from the 10th week. Similar to NE's findings, it is evident that higher variance in V-Q curves corresponds to greater battery degradation and shorter lifespan. On the right side of Figure 2b, the relationship between the variance of cross-difference V-Q curves and the difference in battery lifespan is displayed, with a random LCO battery as the reference cell. It's important to note that the variance here is signed due to the dependency of the difference curves between two batteries on which one serves as the reference. Similar to self-difference, it can be observed that higher variance in V-Q curves indicates larger differences in lifespan between two batteries, implying strong correlation. In practice, we utilize complete V-Q curves as inputs rather than their variances to allow the neural network to capture more comprehensive information.

\figurename~\ref{fig:pipeline}b visually demonstrates the relationship between voltage-capacity curves and battery lifetime based on two different reference signals. The upper of \figurename~\ref{fig:pipeline}b shows that the area between the IntraCD curves is highly correlated with the battery lifetime, where a larger area indicates a worse battery degradation and thus a shorter lifetime~\cite{NE}. The lower of \figurename~\ref{fig:pipeline}b depicts that a larger area of InterCD curves calculated between different battery types also suggests a larger lifetime difference, as it reflects the difference in their state of health. In this way, the target lifetime is implied by the InterCD features when using a reference cell with known lifetime. Note that while the IntraCD displays a linear relationship with the battery lifetime, the InterCD features and the lifetime difference is clearly non-linear and thus requires stronger models for pattern recognition.
% In practice, we utilize the six complete capacity-indexed curves as inputs rather than the areas to allow better flexibility in capturing more complex patterns.

Approaches based on IntraCD often necessitate careful early stopping to prevent potential overfitting in data-scarce scenarios.
In contrast, $N(N-1)$ ordered input pairs can be constructed from $N$ batteries to significantly enhance training data utilization for InterCD-based methods.
% In contrast, the cross-difference-based approaches can harness the interrelation between batteries, enable more effective data utilization, and result in enhanced predictive accuracy and robustness.
Moreover, we can utilize a group of reference cells for one target cell and take the ensemble of their predictions to further improve the inference performance.
Note that the performance enhancement achieved through the ensemble of reference cells is a unique advantage of InterCD, and is orthogonal to other techniques such as data augmentation and model ensembles.

Moreover, we notice that the IntraCD- and InterCD-based models actually learns from different patterns to predict equivalent targets.
% We notice that the input spaces of self-diff and cross-diff are consistent and both methods map to the same linear space.
Therefore, it is beneficial to align the embedding spaces of the two methods and make them share information with each other.
In this way, IntraCD and InterCD can act as mutual regularization and both converge to better solutions.
Specifically, we employ separate encoders with the same architecture to capture the distinct patterns in IntraCD and InterCD features, as show in \figurename~\ref{fig:pipeline}c.
% We adopt the same architecture for the two encoders to ease the embedding space alignment.
Both encoders map the features to an aligned embedding space, and a shared linear regression layer produces either the predictions of the battery lifetime or estimations of lifetime differences for the two branches.
Through this shared regression layer, we can connect the optimization of self- and cross-difference-based predictors and enjoy their mutual complementarity for better predictive performance.
The result framework, named the \textit{deep contrastive battery lifetime prediction} (DCBLP) framework, outperforms the established methodologies by a large margin on various test datasets, which we detail in the following section.

\subsection{Comprehensive Benchmark Comparison}

\begin{table*}[!t]
\footnotesize
\begin{tabular}{lllllllllllll}
\toprule
{\multirow{2}{*}{Method}} & \multicolumn{2}{c}{MATR-1} & \multicolumn{2}{c}{MATR-2} & \multicolumn{2}{c}{MATR-full} & \multicolumn{2}{c}{HUST} & \multicolumn{2}{c}{MIX-20} & \multicolumn{2}{c}{MIX-100} \\
{} &    RMSE & MAPE(\%) &     RMSE & MAPE(\%) &      RMSE & MAPE(\%) &    RMSE & MAPE(\%) &     RMSE & MAPE(\%) &    RMSE & MAPE(\%) \\
\midrule
Training Mean                 &     399 &      28 &      511 &      36 &       331 &      31 &     420 &      18 &      593 &     102 &     573 &      59 \\
\midrule
``Variance'' Model\cite{NE}        &     138 &      15 &      196 &      12 &       179 &      17 &     398 &      17 &      601 &      95 &     521 &      39 \\
``Discharge'' Model\cite{NE}       &      \underline{86} &       \underline{8} &      \underline{173} &      \underline{11} &       144 &      14 &     \underline{322} &      \underline{14} &  >2000 &    >100 &    1743 &      47 \\
``Full'' Model\cite{NE}            &     100 &      11 &      214 &      12 &       \underline{139} &      14 &     335 &      14 &      441 &      53 &     331 &      22 \\
Ridge Regression\cite{attia2021statistical}      &     125 &      13 &      188 &      11 &       178 &      13 &    1047 &      36 &      806 &     150 &     395 &      30 \\
PCR\cite{attia2021statistical}                   &     100 &      11 &      176 &      11 &       173 &      13 &     435 &      19 &      701 &      78 &     384 &      28 \\
PLSR\cite{attia2021statistical}                  &      97 &      10 &      193 &      11 &       168 &      13 &     431 &      18 &      543 &      77 &     371 &      26 \\
SVM Regression        &     140 &      15 &      300 &      18 &       145 &      \underline{11} &     344 &      16 &      438 &      46 &     257 &      18 \\
Random Forest\cite{attia2021statistical}         &     140 &      15 &      202 &      11 &       203 &      16 &     348 &      16 &      \underline{288} &      \underline{31} &     \underline{211} &      \underline{14} \\
\midrule
MLP\cite{attia2021statistical}                   &   162±7 &    12±0 &    207±4 &    11±0 &     165±5 &    12±1 &   444±5 &    18±1 &   532±25 &    61±6 &  455±37 &    27±1 \\
LSTM                  &  123±11 &    12±2 &   226±36 &    14±2 &    200±21 &    14±1 &  442±32 &    20±1 &   417±62 &    37±7 &  266±11 &    15±1 \\
CNN\cite{attia2021statistical}                   &  115±96 &     9±6 &  237±107 &    17±8 &    223±72 &    15±3 &  445±35 &    21±1 &  785±132 &    41±4 &  261±38 &    15±1 \\
\midrule
InterCD &    73±3 &     7±0 &   260±13 &    17±1 &     109±7 &    10±1 &  265±10 &    10±1 &   210±15 &    18±1 &  181±13 &    12±1 \\
DCBLP                 &    \textbf{59±2} &     \textbf{6±0} &   \textbf{163±12} &    \textbf{11±1} &      \textbf{85±8} &     \textbf{7±1} &   \textbf{264±9} &    \textbf{10±1} &   \textbf{201±18} &    \textbf{18±1} &   \textbf{158±7} &    \textbf{10±0} \\
\bottomrule
\end{tabular}
\caption{Comparison results with baseline methods. We employ bold font to emphasize the best-performing method and utilize underlines to denote the second-best baselines. For neural-network-based methods, we report the mean and standard deviation of eight seeds.}
\label{tab:main}
\end{table*}

\begin{figure*}[!t]
    \includegraphics[width=0.8\linewidth]{images/fig2.5.pdf}
    \caption{Visualization of comparison results. \textbf{a}: Performance of NN-based methods using different random seeds. CNN model exhibits larger variance than LSTM but sometimes achieves smaller errors. DCBLP is more accurate and robust to all baseline models. \textbf{b}: Prediction error for individual battery cells of \texttt{MIX-100} dataset. \textbf{c}: Cumulative absolute error plotted with respect to the fraction of test samples used from \texttt{MIX-100} dataset. Stronger models are those closer to the upper-left corner.}
    \label{fig:comparison}
\end{figure*}

We curated, to the best of our knowledge, all the existing battery data suitable for early cycle battery life prediction to comprehensively evaluate our method in comparison with existing approaches.
Six distinct test datasets covering various of battery models and operating conditions are constructed for experimentation.

\texttt{MATR-1} and \texttt{MATR-2}~\cite{NE} consist of $123$ commercial 18650 lithium-ion phosphate/graphite (LFP) batteries.
All batteries share the same discharging protocol but are charged at different rates.
\texttt{MATR-2} requires the model to generalize to different charging protocols while the training and test dataset of \texttt{MATR-1} follow the same distribution.
We construct \texttt{MATR-full} that includes all the batteries from \texttt{MATR-1} and \texttt{MATR-2}, as well as additional $55$ LFP 18650 cells cycled with the optimized charging protocols~\cite{CLO} to assess how the model generalizes across diverse data batches obtained at different time points.
The \texttt{HUST} dataset~\cite{HUST} involves $77$ LFP batteries with a constant charging protocol but different discharge speeds.
All the cells in these four datasets belong to the same battery model.

Additionally, we collected batteries used in prior studies including CALCE~\cite{CALCE1,CALCE2,CALCE3}, HNEI~\cite{HNEI}, UL-PUR~\cite{ULPUR}, RWTH~\cite{RWTH} and SNL~\cite{SNL}.
By combining these batteries with \texttt{MATR-full} and \texttt{HUST}, we obtained a total collection of 401 batteries.
To evaluate the performance under different lifetime prediction scenarios, we developed two test datasets \texttt{MIX-20} and \texttt{MIX-100}.
In \texttt{MIX-20}, the models are required to predict the cycles before degradation to 90\% of the nominal capacity, using the data from only the first 20 cycles.
In \texttt{MIX-100}, the models predict the 80\% end of life point using data from the first 100 cycles.
Notably, batteries that had already degraded to the end of life during the early cycles were excluded in the experiments.

As \figurename~\ref{fig:dataset}a shows, the collected dataset exhibits a more comprehensive coverage that goes beyond the confines of previous works. This diversity requires the model to capture and distinguish the degradation patterns caused by various factors for generalization. \figurename~\ref{fig:dataset}b visualizes the battery capacity degradation in the first $1500$ and $100$ cycles of the batteries. We can see that the degradation is highly non-linear and varies significantly between batteries. Also, the degradation within the first 100 cycles is often imperceptible for a significant number of batteries. As a result, a substantial portion of batteries exhibit similar degradation speed, making it challenging to discern the extent of ageing. For more comprehensive details on dataset construction, please refer to the Supplementary Information.

\begin{figure*}[!t]
    \includegraphics[width=\linewidth]{images/new_fig4_bar.pdf}
    \caption{Ablation studies. \textbf{a}: Enhanced predictive performance necessiates the inclusion of the complete voltage and current signals, as well as their interactions, from both charging and discharging stages. Here the derived interaction features refer to the differential voltage-capacity curve and resistance-capacity curve. \textbf{b}: Intra-cell difference model is prune to overfitting while inter-cell difference model and DCBLP exhibit robust convergence. \textbf{c}: Leveraging the inherent advantages of both intra- and inter-cell difference models, DCBLP achieves superior performance over their combined ensemble.}
    \label{fig:ablation}
\end{figure*}

Table~\ref{tab:main} presents the comparison results of the proposed methods against various baselines on these six datasets.
Employing only the InterCD method achieves superior performance on \texttt{MATR-1}, \texttt{MATR-full} and \texttt{HUST}.
This means the model effectively captures the degradation patterns of the LFP cells under different charging and discharging protocols.
InterCD shows even larger performance advantage in comparison with the baselines on \texttt{MIX-20} and \texttt{MIX-100}.
This phenomenon arises due to the tendency of the IntraCD-based baselines to underfit or even diverge as they encounter an increasing variety of battery types.
In contrast, the InterCD adeptly captures the diverse degradation patterns, thus yielding more accurate predictions.
We observe a suboptimal performance of the InterCD method on \texttt{MATR-2}.
Further investigation indicates that the cause is several outlier battery cells that resemble the electrical signals  of batteries with a much smaller lifetime.
We leave the detailed analysis to the Supplementary Information. 

With the co-training IntraCD and InterCD, DCBLP further shows a significant performance boost over InterCD alone, leading to the best predictive performance on all datasets.
It is important to note that, no method prior to DCBLP has managed to consistently achieve optimal performance across all datasets.
DCBLP reduced the relative RMSE by $31.4\%$, $5.8\%$, $38.8\%$, $18.0\%$, $30.2\%$, $25.11\%$ respectively on the six datasets over the the second-best baselines.
DCBLP also achieved $\leq 18\%$ MAPE on all datasets, meaning that DCBLP predicts relatively small errors for all cells under diverse prediction scenarios.
In contrast, the baseline methods can produce $>30\%$ relative errors, rendering them unsuitable for general applications.
% This suggests that the advantage of the proposed methods over the existing methods is likely to be even more pronounced when dealing with a broader scope of battery types and more intricate operational conditions.
% MIX-20 stands as the most challenging dataset, with prediction errors exceeding those for MIX-100 across all methods. However, our approach demonstrates greater improvement relative to the strongest baseline on MIX-20, underscoring its increased efficacy even during early cycles with fewer data points.

% TODO: talk about figure 2.5
\figurename~\ref{fig:comparison}a demonstrates the comparison of deep models under different random seeds on the six datasets. Among the baselines, the multi-layer perceptron (MLP) demonstrates modest prediction errors with the lowest variance on average. The RMSE of the convolutional network (CNN) shows the largest variance, yet achieves the lowest errors in four datasets among the baselines. Note that CNN becomes the strongest baseline when using the optimal seeds, consistent with Ref.~\cite{attia2021statistical}. The long short term memory (LSTM) network achieves the best accuracy-variance trade-off. DCBLP outperforms these baselines in both accuracy and robustness. \figurename~\ref{fig:comparison}b displays the instance-level prediction errors of DCBLP on \texttt{MIX-100} dataset, where the absolute percentage error is lower than $20\%$ for $84.7\%$ cells. The results of other datasets are left to the Supplementary Information. \figurename~\ref{fig:comparison}c plots the cumulative absolute error with respect to the fraction of test samples in \texttt{MIX-100} dataset. The error curves of the random forest (RF) and DCBLP initially coincide for the first approximately $50\%$ of test samples, after which the error of RF begins to escalate at a faster rate than that of DCBLP. This suggests that RF accurately captures the patterns within a subset of the samples, whereas DCBLP excels at capturing the patterns in the remaining portion. Finally, the consistent slope of the error growth curve for DCBLP signifies that DCBLP does not exhibit excessively large prediction errors for any batteries.

We conduct further ablation experiments to study the components of DCBLP.
\figurename~\ref{fig:ablation}a shows the performance of DCBLP when using a subset of the six capacity-indexed features.
It's evident that all six features play a crucial role in achieving improved predictive performance. 
Current features can lead to high variance and large errors, yet they are necessary for \texttt{MIX-20}. Voltage and discharge features demonstrate strong performance across all datasets. Merging voltage and current features from both charge and discharge stages results in enhanced performance, with the best outcomes achieved by employing all six features.

\figurename~\ref{fig:ablation}b illustrates the convergence of IntraCD, InterCD, and DCBLP during training on \texttt{MIX-100}.
We observed that the IntraCD model quickly reaches a low error at the 200-th epoch but then starts to overfit.
As training progresses, the variance between different seeds of IntraCD gradually intensifies and the models continue to diverge.
In practice, without additional validation samples for early stopping due to the data scarcity issue, the IntraCD-based methods demonstrate poor robustness and are very sensitive to initialization.
In contrast, the InterCD-based method gradually converge during training without overfitting, irrespective of the random seed employed.
This highlights the robustness of the InterCD-based method, although its final regression error is slightly larger than the lowest error of the IntraCD-based method.
Owing to the co-training of the both branches, DCBLP combines the advantages of both branches and robustly converges to a more accurate solution.

\figurename~\ref{fig:ablation}c presents the ablation experiments with different reference signals.
Across all datasets, IntraCD difference methods exhibit the highest error and variance due to its weak robustness during training.
The InterCD shows good robustness with lower variance across all datasets, yet its prediction accuracy is slightly lower than that of the IntraCD on some datasets, as its predictions are implicitly derived through the reference cells.
The ensemble of the two branches obtains better performance on \texttt{HUST} and \texttt{MIX-100}, yet on other datasets it inherits the flaws of either branch, resulting in higher variance or suboptimal accuracy.
DCBLP achieved the most robust and precise lifetime estimation across all datasets, demonstrating that through the co-training with shared prediction layers, the model better integrates the strength of both branches and yields the strongest predictive performance.

\begin{figure*}[!t]
    \includegraphics[width=\linewidth]{images/fig4.pdf}
    \caption{Study of reference cells. \textbf{a}: The predictive error of different choices for reference cell. \textbf{b}: The predictive error decreases when increasing the number of reference cells for a single target battery. \textbf{c}: The inference time and batch size of DCBLP can support real-time lifetime prediction applications.}
    \label{fig:reference}
\end{figure*}

Unlike IntraCD-based methods, which can only use its own cycle as reference signals, InterCD methods allow flexible selection of different batteries as references.
This additional freedom enables us to enhance the predictive performance through the careful choice of reference cells.

\figurename~\ref{fig:reference}a demonstrates the substantial impact of different reference cell selection strategy on the prediction error for each battery for InterCD.
% We can see that the difference between the best and the worst reference choices can exceed an absolute error of $1500$ cycles.
The gap between the least favorable and optimal reference choices can lead to an absolute error exceeding $1500$ cycles.
For DCBLP, we employ the ensemble of the reference cells by their median prediction as the final prediction. Impressively, this choice leads to a significant improvement compared to the worst-case scenario, resulting in an absolute error reduction of more than $1000$ cycles for specific cells.
However, a substantial gap still exists between the median choice and the optimal one.
Closing this gap requires the model to intelligently select the most suitable reference cell for each battery.
We provide more analysis into this issue in the Supplementary Materials, and the search for the optimal reference choice is deferred to future work.

\figurename~\ref{fig:reference}b illustrates the relationship between the number of reference cells and the prediction error of InterCD.
As the number of reference cells increases, both the average prediction error and the variance between different random seeds decrease.
% Increasing the number of reference cells results in a decrease in both the prediction error and the variance among different random seeds.
This indicates that a larger number of reference cells simultaneously enhances the model's accuracy and robustness.
\figurename~\ref{fig:reference}c depicts the impact of the reference cell count on the inference speed and batch size for DCBLP.
With an increase in reference size, there is a corresponding rise in inference time and a reduction in batch size.
A large number of reference cells leads to higher computational cost.
However, even with a very large reference size of $64$ for each cell, the inference speed of the model remains notably fast, operating at $178.8$ cells per second.
This underscores the capability of DCBLP as a real-time predictor for battery lifetime.
Moreover, \figurename~\ref{fig:reference} also demonstrates that the performance improvement brought by more reference cells gradually saturates as the reference size increases.
We can conclude that DCBLP can achieve a desirable balance of efficiency, performance, and robustness with a moderate size of reference cells.
% Considering \figurename~\ref{fig:reference} alongside, when utilizing an appropriately size of reference cells, DCBLP achieves a very good balance of efficiency, performance, and robustness.

